A survey on quasi-isometries of pairs: invariants and rigidity

This survey studies pairs $(G,\mathcal{P})$ with $G$ a finitely generated group and $\mathcal{P}$ a (finite) collection of subgroups of $G$. We explore the notion of quasi-isometry of such pairs and the notion of a qi-characteristic collection of subgroups. Both notions are abstractions of phenomena that have appeared repeatedly in the work of several people within the quasi-isometric rigidity realm.

==> old_todo.tex <==
\section{To do list}


\subsection{Independence of conditions in the qi-characteristic definition}

 \begin{example}
 \label{NonExamples}   The following examples illustrate that conditions (1)-(3) in \Cref{def:qicharacteristic} are independent of each other.  
 \begin{enumerate} 
\item \label{Example01} Consider the pair $(X, \mathcal{A})$ where $X$ is the $n$-dimensional Euclidean space and $\mathcal{A}$ consists of a single compact subset of $X$. Note that  any quasi-isometry $q\colon X \to X$ is a quasi-isometry of the pair $q\colon (X, \mathcal{A})  \to (X, \mathcal{A})$. On the other hand, the collection $\mathcal{A}$ is not qi-characteristic in $X$, the first condition fails by considering translations,  while the  conditions (2) and (3) hold.

\item Let $X=\mathbb H^n$ be the n-dimensional hyperbolic space and let $\mathcal A$ be the set of all geodesic lines in $X$. Then condition (2) does not hold while conditions (1) and (3) hold. Condition (1) holds because $\mathbb{H}^n$ is a hyperbolic space in the sense of Gromov.

\item Let $X$ be the real line and let $\mathcal{A}=\{ \{n\} \colon n\in \Z \}$. Then conditions $(1)$ and $(2)$ hold, but $(3)$ does not.
\end{enumerate}
 \end{example}
 
\subsection{}


\begin{enumerate}
    \item Eduardo and Luis qi characteristic paper \cite{MaSa21}. \commentL{Done?}
    
    \item Eduardo, Sam and Luis paper qi invariance of Dehn functions \cite{HuMaSa21}. \commentL{Done?}
    
    \item ordinary finiteness properties $F_n$, $FP_n$ (we can give a proof!) \commentS{done}
    
    \item Anthony Genevois papers \cite{G19} on qi characteristic collections in Coxeter groups. \commentL{Done}
    
    \item Anthony Genevois and Romain Tessera \cite{GT21} about qi characteristic of lamplighter groups. \commentL{Done}
    
    \item Mention Schwartz paper, where the qi-characteristic collections first appeared (pressumably). Kapovich, Kevin White, Lafont-Frigerio-Sisto.
    
    \item Hruska's work on quasi-isometry of pairs. \commentL{Done?}
    
    \item Alexander Margolis' work. \commentS{done}
    
    \item JSJ decompositions, try to link it with qi rigidity of pairs. \commentL{Does this have to do with Papasoglu's paper \cite{Pa05}?}
    
    \item Kapovich-Leeb work on qi rigidity. \commentL{Done} 
    
    \item Mosher-Sageev-White work on qi-rigidity. \commentL{I am not very sure what work is this one...}
    
    \item Papasoglu work on qi-rigidity.
    
    \item Osin's work on relatively hyperbolic groups and linear Dehn relative functions. Toghether with Drutu-Mosher's paper they prove that linear relative Dehn functions are qi-invariants of pairs.
    
    \item Raise questions about qi-invariants of pairs and qi-rigidity phenomena.
\end{enumerate}



Ideas for questions:

\begin{question}
What properties of a pair $(G,\calp)$ are invariant under quasi-isometries of pairs?
\end{question}

\begin{question}
When is a collection of hyperbolically embedded subgroups of a group $G$ qi-characteristic?  Note something about MCGs which I can't remember (maybe that pseudo-Ansovos are not qi-char. but that MCG is qi rigid?).
\end{question}

Every quasi-isometry of the mapping class group is at uniform distance from left multiplication by an element, see Theorem 1.1 in section 10 of 
Jason Behrstock. Bruce Kleiner. Yair Minsky. Lee Mosher. "Geometry and rigidity of mapping class groups." Geom. Topol. 16 (2) 781 - 888, 2012.
This means that the hyperbolically embedded subgroup generated by a pseudo-Anosov is qi-characteristic.   Moreover, one can have a collection of maximal virtually cyclic subgroups each generated by a pseudo-Anosov, and the collection is hyperbolically embedded and qi-characteristic.   Such a collection, I believe, can always be extended by adding a new subgroup generated by a pseudo-Anosov in "different direction", so one can create an increasing sequence of finite q.i characteristic hyperbolically embedded collections. Even, maybe the collection of all maximal virtually cyclic subgroups generated by pseudo-Anosovs might be "qi-characteristic"

\begin{question}
What is a characterisation of the class of groups with a well-defined relative Dehn function with respect to a non-trivial collection?
\end{question}

\begin{question}
For non-solvable Baumslag-Solitar groups is the subgroup generated by the stable letter qi-characteristic?
\end{question}


